ChronoSteer: Bridging Large Language Model and Time Series Foundation Model via Synthetic Cross-Modal Alignment Dataset

Conventional forecasting methods are trained end-to-end on unimodal time series, which limits their ability to exploit textual information and undermines their generalization in data-scarce scenarios. Recently, large language models (LLMs) and time series foundation models (TSFMs) have demonstrated powerful capabilities in complex textual reasoning and zero-shot temporal modeling, respectively. Integrating these strengths to construct a multimodal time series foundation model that jointly leverages temporal and textual information for zero-shot future inference has emerged as a promising research direction. However, the scarcity of large-scale, high-quality multimodal datasets remains a fundamental obstacle. To address this challenge, we propose ChronoSteer, a decoupled agentic framework that learns cross-modal alignment from synthetic paired supervision. Specifically, a pretrained LLM first converts textual events into revision instructions that steer the initial unimodal prediction produced by a frozen TSFM. These revision instructions form an intermediate instruction space that bridges the semantic gap between text and time series while fully leveraging pretrained knowledge. Technically, the instructions are discretized into a compact codebook of instruction anchors, effectively mitigating semantic divergence while reducing the cost of dataset construction. Finally, we adopt a two-stage training strategy to recover the fine-grained magnitude information lost during discretization. Furthermore, we release a leakage-controlled multimodal benchmark constructed with temporal separation and textual context available before the prediction window. When paired with an LLM and trained on synthetic cross-modal alignment data, ChronoSteer achieves a 25.8% improvement in zero-shot prediction accuracy over its unimodal backbone, and outperforms prior state-of-the-art unimodal and multimodal ...

==> table/noise_analysis.tex <==
\begin{tabular}{@{}c|c|cccccc@{}}
	\toprule
	\multirow{2}{*}{Method}                     & \multirow{2}{*}{Noise} & \multicolumn{2}{c}{Energy} & \multicolumn{2}{c}{Traffic} & \multicolumn{2}{c}{Weather}                                                       \\ \cmidrule(l){3-8}
	                                            &                        & MSE                        & MAE                         & MSE                         & MAE             & MSE             & MAE             \\ \midrule
	\multirow{6}{*}{\rotatebox{90}{Unimodal}}   & 0.00                   & 0.699$\pm$0.000            & 0.262$\pm$0.000             & 0.545$\pm$0.000             & 0.509$\pm$0.000 & 1.581$\pm$0.000 & 0.956$\pm$0.000 \\ \cmidrule(l){2-8}
	                                            & 0.05                   & 0.703$\pm$0.008            & 0.261$\pm$0.003             & 0.546$\pm$0.011             & 0.504$\pm$0.008 & 1.591$\pm$0.017 & 0.961$\pm$0.017 \\
	                                            & 0.10                   & 0.707$\pm$0.011            & 0.263$\pm$0.003             & 0.547$\pm$0.005             & 0.517$\pm$0.005 & 1.595$\pm$0.024 & 0.962$\pm$0.014 \\
	                                            & 0.15                   & 0.715$\pm$0.009            & 0.267$\pm$0.003             & 0.559$\pm$0.009             & 0.519$\pm$0.004 & 1.607$\pm$0.025 & 0.971$\pm$0.010 \\
	                                            & 0.20                   & 0.716$\pm$0.009            & 0.273$\pm$0.004             & 0.562$\pm$0.009             & 0.527$\pm$0.008 & 1.619$\pm$0.030 & 0.997$\pm$0.014 \\
	                                            & 0.25                   & 0.729$\pm$0.009            & 0.274$\pm$0.004             & 0.568$\pm$0.005             & 0.529$\pm$0.005 & 1.622$\pm$0.026 & 1.020$\pm$0.014 \\ \midrule
	\multirow{6}{*}{\rotatebox{90}{Multimodal}} & 0.00                   & 0.575$\pm$0.010            & 0.257$\pm$0.003             & 0.381$\pm$0.004             & 0.430$\pm$0.003 & 0.996$\pm$0.015 & 0.738$\pm$0.013 \\ \cmidrule(l){2-8}
	                                            & 0.05                   & 0.576$\pm$0.008            & 0.261$\pm$0.004             & 0.385$\pm$0.005             & 0.431$\pm$0.007 & 1.005$\pm$0.009 & 0.741$\pm$0.012 \\
	                                            & 0.10                   & 0.583$\pm$0.006            & 0.262$\pm$0.004             & 0.390$\pm$0.004             & 0.438$\pm$0.007 & 1.014$\pm$0.018 & 0.741$\pm$0.008 \\
	                                            & 0.15                   & 0.586$\pm$0.007            & 0.263$\pm$0.002             & 0.392$\pm$0.006             & 0.443$\pm$0.004 & 1.018$\pm$0.015 & 0.756$\pm$0.012 \\
	                                            & 0.20                   & 0.587$\pm$0.011            & 0.265$\pm$0.003             & 0.399$\pm$0.005             & 0.451$\pm$0.006 & 1.023$\pm$0.017 & 0.761$\pm$0.013 \\
	                                            & 0.25                   & 0.594$\pm$0.009            & 0.267$\pm$0.004             & 0.403$\pm$0.004             & 0.451$\pm$0.007 & 1.029$\pm$0.013 & 0.767$\pm$0.009 \\ \bottomrule
\end{tabular}
